Automated Harmfulness Testing for Code Large Language Models

Generative AI systems powered by Large Language Models (LLMs) usually use content moderation to prevent harmful content spread. To evaluate the robustness of content moderation, several metamorphic testing techniques have been proposed to test content moderation software. However, these techniques mainly focus on general users (e.g., text and image generation). Meanwhile, a recent study shows that developers consider using harmful keywords when naming software artifacts to be an unethical behavior. Exposure to harmful content in software artifacts can negatively impact the mental health of developers, making content moderation for Code Large Language Models (Code LLMs) essential. We conduct a preliminary study on program transformations that can be misused to introduce harmful content into auto-generated code, identifying 32 such transformations. To address this, we propose CHT, a coverage-guided harmfulness testing framework that generates prompts using diverse transformations and harmful keywords injected into benign programs. CHT evaluates output damage to assess potential risks in LLM-generated explanations and code. Our evaluation of four Code LLMs and GPT-4o-mini reveals that content moderation in LLM-based code generation is easily bypassed. To enhance moderation, we propose a two-phase approach that first detects harmful content before generating output, improving moderation effectiveness by 483.76\%.

==> datasettable.tex <==
\begin{table*}[h]
\caption{Datasets for Code Generation}
\label{tab:dataset}
\resizebox{\textwidth}{!}{
\begin{tabular}{|l|p{2cm}|p{2cm}|p{2cm}|p{2cm}|p{2cm}|p{3cm}|}
\hline
\small
Benchmark &
  Natural Languages &
  Programming Languages &
  Supported Tasks &
  Size &
  Test case &
Unique Features \\ \hline
APPS~\cite{hendrycks2021measuring} &
  English &
  Python &
  Text-code &
  10,000 problems &
  130,000 total test cases &
  One of the earlier dataset with crowd-sourced   questions for program synthesis \\ \hline
HumanEval~\cite{chen2021evaluating} &
  English &
  Python &
  Text-code &
  164 problems &
  Average 7.7 tests per problem &
  Handwritten problems to evaluate   functional correctness and measure problem-solving capabilities \\ \hline
MBPP~\cite{austin2021program} &
  English &
  Python &
  Text-code &
  974 python functions &
  3 test cases for each problem &
  Measure the ability of these models to   synthesize short Python programs \\ \hline
CONCODE~\cite{iyer2018mapping} &
  English &
  Java &
  Text-code &
  100,000   (classes, NL, code) tuples &
  No test &
  Classes from diverse domains\\ \hline
PandasEval, NumpyEval~\cite{zan2022cert} &
  English &
  Python &
  Text-code &
  101 programming problems &
  20 tests for each problem &
  Library-oriented code generation \\ \hline
%CODEXGLUE~\cite{DBLP:journals/corr/abs-2102-04664} &  English &  6 languages & 10 tasks &  113 programming tasks from recent contests, 335 incorrect   solutions &  1-3 public tests for each problem &   Collection of datasets that supports 10 programming language understanding and generation tasks.\\ \hline
MCoNaLa~\cite{wang2022mconala} &
  Spanish, Japanese, and Russian &
  Python &
  Text-code & 
  896 NL-Code pairs & No test
   &
  Support several natural languages beyond English \\ \hline
LLMDefects~\cite{fan2023automated} &
  English &
  Java &
  Text\&code-code &
  113 programming tasks from recent contests, 335 incorrect   solutions &
  1-3 public tests for each problem &
  Contains mistakes in code generated by LLMs.\\ \hline
ClassEval~\cite{du2023classeval} &
  English &
  Python &
  Text-code &
  100 tasks &
  Contain method-level and class-level   tests &
  Class-level code generation \\ \hline
AixBench~\cite{hao2022aixbench} &
  English, Chinese &
  Java &
  Text-code &
  175 samples for automated Test, 161 NL   Task Description &
  Contain hand-crafted tests &
  Contain hand-crafted automated test   cases \\ \hline
  MultiPL-E~\cite{multiple} &
  English &
  19 languages (e.g., Julia, Swift) &
  Text-code &
  161 problems from HumanEval~\cite{chen2021evaluating}, 974 from MBPP~\cite{austin2021program}  &
  Use tests from prior benchmarks~\cite{chen2021evaluating,austin2021program} &
  Extend HumanEval~\cite{chen2021evaluating} and
MBPP~\cite{austin2021program} to 18 languages by translating programs and unit tests\\ \hline
SWE-Bench~\cite{jimenez2023swe} &
  English &
  Python &
  Text\&code-code&
  2294 problems from 12 projects &
  Average 120.8 total tests for each problem &
  Evaluate the ability to resolve real-world GitHub\\ \hline
CodeScope~\cite{yan2023codescope} &
  English &
  43 languages &
  8 tasks&
  200--5,382 samples for each task &
  Contain tests for some tasks &
  Evaluate generated code on difficulty, efficiency,
and length\\ \hline
NoFunEval~\cite{singhal2024nofuneval} &
  English &
  Python, Java, C, JavaScript, Kotlin&
  Text\&code-code, classify correctness &
  47--397 samples for each task &
  No test &
  Evaluate non-functional requirements (latency, security, efficiency)\\ \hline
LiveCodeBench~\cite{jain2024livecodebench} &
  English &
  Python &
  Text\&code-code &
  Collect new problems over time &
  Use tests from programming problems or LLM-generated tests &
  Mitigate contamination issues by crawling new problems\\ \hline
\end{tabular}}
\end{table*}

==> different-related.tex <==

\iffalse

\begin{table}[t]
\centering
\caption{Differences with relevant work that aim to produce reduced programs}
\vspace{-3pt}
\small
\label{tab:Differences}

\begin{tabularx}{\columnwidth}{>{\hsize=.19\hsize}X|>{\hsize=.27\hsize}X|>{\hsize=0.20\hsize}X|>{\hsize=.35\hsize}X|>{\hsize=0.15\hsize}X}
\hline
Approach & Simplification Goals & Transformations & Simplification Technique & Tests \\ \hline
Delta Debugging$^D$ & Debugging, test input minimization, feature isolation & Deletion & Delta debugging~\cite{zeller2001automated, ddmin,ddinput}, hierarchical delta debugging~\cite{misherghi2006hdd, hodovan2017coarse} & Need to run tests \\ \hline
Program Reduction$^D$ & Test case minimization & Deleting bug-irrelevant elements & Perses~\cite{sun2018perses}, Vulcan~\cite{xu2023pushing} & Need to run tests \\ \hline
Program Slicing$^D$  & Debugging, testing, software maintenance & Statements with control or data dependency; Deletion* & Dependency Analysis~\cite{wang2008dynamic,agrawal1990dynamic,harman1995using,lu2012automatic,binkley2013observation} & May/May not run tests \\ \hline
Program Debloating$^D$  & Reduce attack surfaces & Deletion & Combine with delta debugging~\cite{heo2018effective}, Dependency Analysis~\cite{qian2019razor} & Need to run tests \\ \hline \hline
Simplication in GP$^R$  & Enforce explanability of models & Rule-based Transformations & Simplification Rules (e.g., algebraic, numerical)~\cite{wong2007effects,javed2022simplification} & May/May not run tests \\ \hline
Refactoring$^R$  & Software maintenance & Rule-based Transformations & Rules based on refactoring types~\cite{zhang2013practical,nievergelt1965automatic,ddinput,jiang2017simplydroid,rabin2021understanding,zeller2001automated,tsantalis2020refactoringminer,Tsantalis:ICSE:2018:RefactoringMiner} & May/May not run tests \\ \hline \hline
Our Work & Generate \simpli{} & Diverse Transformations & Based on deep learning and LLMs  & Need to run tests \\ \hline
\end{tabularx}
{\raggedright Approaches marked with $^D$ 
 represents deletion-based approaches, whereas approaches marked with $^R$ denotes rule-based approaches. *We consider program slicing as a deletion-based approach that removes statements without dependency from the original program. \par}
\end{table}



\fi








%TODO: change in camera ready

{
\begin{table*}
\centering
\caption{\modify{Differences with existing work}}
\label{tab:Differences}
\small
\setlength{\tabcolsep}{0.3em}
\begin{adjustbox}{width=\linewidth}
{\color{modifyc}\begin{tabular}{|p{4cm}|p{4.5cm}|p{4.5cm}|p{4.5cm}|p{4.5cm}|}
\hline
\textbf{Related Approach} & \textbf{Definitions/Goals} & \textbf{Attributes} & \textbf{Technique} & \textbf{Types of software} \\ \hline
Fairness testing~\cite{10.1145/3652155,galhotra2017fairness,asyrofi2021biasfinder} & Reveal fairness bugs (software discrimination across \textbf{groups}) through code execution & social groups (e.g., race, gender, age) & \textbf{Metamorphic testing} based on input pairs that differ in \textbf{group attributes} (e.g., demographic bias like gender, occupation, country-of-origin~\cite{asyrofi2021biasfinder}) & Mostly focus on \textbf{text generation} and \textbf{image generation} \\ \hline
Bias detection~\cite{chakraborty2021bias,lin2024investigating,DBLP:conf/cvpr/NiuTZL0W21,DBLP:conf/kdd/WeiFCWYH21,asyrofi2021biasfinder} & Detect bias across \textbf{groups} & social groups (e.g., race, gender, age), popularity bias & 
\textbf{Empirical evaluation} and \textbf{study} & machine learning software (e.g., sentiment analysis systems~\cite{asyrofi2021biasfinder}) \\ \hline
Study of GenAI (e.g., ChatGPT~\cite{10.1016/j.ijinfomgt.2023.102700,DBLP:journals/corr/abs-2112-04359,articlegpt}) & Discuss potential risks~\cite{DBLP:journals/corr/abs-2112-04359} and bias~\cite{articlegpt} & various risks and bias & \textbf{Literature review} and \textbf{study} & AI-driven software \\ \hline
AI ethics \textbf{guidelines}~\cite{jobin2019global,correa2023worldwide} & Discuss potential risks~\cite{DBLP:journals/corr/abs-2112-04359}, bias~\cite{articlegpt}, and provide ethics guidelines (with up to 11 clusters of principles) & 11 clusters of principles include transparency, justice and fairness, non-maleficence, responsibility, privacy, beneficence, freedom and autonomy, trust, sustainability, dignity, and solidarity. & - & AI-driven software \\ \hline
Adversary Prompting~\cite{systemfourcard,systemocard,trustai,kumar2023certifying,zou2023universal}/examples~\cite{DBLP:journals/corr/GoodfellowSS14,9825895} & Form inputs by applying small but \textbf{intentionally worst-case} perturbations to examples from the dataset. & security-related attributes for planning attacks, hate speech, social groups (e.g., race, gender, age) & Use adversarial mindset to \textbf{manually perform} attacks via experts (``red teaming'')~\cite{systemfourcard,systemocard,trustai} or automatically add \textbf{small perturbations} (e.g., rotation~\cite{DBLP:journals/corr/GoodfellowSS14}) & Mostly focus on \textbf{text generation} and \textbf{image generation} \\ \hline
%Adversary prompting~\cite{systemfourcard,systemocard,trustai} & Planning attacks& security-related attributes for planning attacks, hate speech, social groups (e.g., race, gender, age) & Use adversarial mindset to \textbf{manually perform} attacks via experts (``red teaming'')~\cite{systemfourcard,systemocard,trustai}  & Mostly focus on \textbf{text generation} and \textbf{image generation} \\ \hline
Ethics testing & Reveal \textbf{unethical behavior} through code execution & \textbf{unethical behavior} that violates corresponding \textbf{ethical principles} (e.g., 4 types of harms defined in taxonomy of harmful content) & \textbf{Systematic testing} guided by ethical principles and taxonomy of harms, program transformations & GenAI software (first to focus on \textbf{software maintenance} tasks, including code generation and autoamted requirement description generation) \\ \hline
\end{tabular}}
\end{adjustbox}
%\begin{tablenotes}
%\footnotesize
%%\item{ \footnotesize
%Approaches marked with $^D$ 
% denotes deletion-based approaches. Approaches marked with $^R$ denotes rule-based approaches. *We consider program slicing as deletion-based as it removes statements without dependency from the original program.
%}
%\end{tablenotes}
\end{table*}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> others.tex <==
\begin{lstlisting}[style=mystyle, escapechar=^,caption=Crash due to transformation issue when joining variable declaration in Eclipse 4.7.1, upquote=true, label={lst:transformation}]
/**
     * ChatGPT generated method to convert to string
     * @param throwable
     * @return 
     */
    private static String convertStackTraceToString(Throwable throwable) {
        StringBuilder result = new StringBuilder();

        // Append the exception message (if any)
        if (throwable.getMessage() != null) {
    result.append(throwable.getClass().getName()).append(": ").append(throwable.getMessage());
            result.append(System.lineSeparator());
        } else {        
    result.append(throwable.getClass().getName()).append(System.lineSeparator());
        }

        // Append each stack trace element
        for (StackTraceElement element : throwable.getStackTrace()) {
            result.append("\tat ").append(element.toString()).append(System.lineSeparator());
        }

        // Append the cause (if any)
        Throwable cause = throwable.getCause();
        if (cause != null) {
            result.append("Caused by: ").append(convertStackTraceToString(cause));
        }
        return result.toString();
    }
}
\end{lstlisting}

==> othertemp.tex <==
\begin{table}[H]
\resizebox{\linewidth}{!}{%
\label{tab:dataset}
\begin{tabular}{|l|r|r|r|}
\hline
Dataset                & Size & Categories/Types_{Ini} & Categories/Types_{Aug} \\  \hline
\cbench &      &                          &                                     \\ \hline
Benign Program Dataset &      &                          &                                     \\ \hline
\end{tabular}}
\end{table}


\begin{table}[]
\resizebox{\linewidth}{!}{%
\label{tab:dataset}
\begin{tabular}{|l|l|l|l|}
\hline
Categories & Gemma~\cite{shieldgemma} & LLama~\cite{inan2023llama} & GPT 4-o~\cite{systemocard} \\ \hline
Doxing                                 &   &   &   \\ \hline
Eating Disorder Promotion              &   &   &   \\ \hline
Extremism, Terrorism \& Organized Crime & Y &   &   \\ \hline
Identity Attack                        &   &   & Y \\ \hline
Identity Misrepresentation             &   & Y & Y \\ \hline
Insult                                 & Y &   &   \\ \hline
Sexual Aggression                      & Y & Y & Y \\ \hline
Threat of Violence                     & Y & Y & Y \\ \hline
Self-Harm                              & Y & Y & Y \\ \hline
Misinformation                         &   &   & Y \\ \hline
Adult Sexual Services                  & Y & Y & Y \\ \hline
Child Sexual Abuse Materials           & Y & Y & Y \\ \hline
Scams                                  &   & Y & Y \\ \hline\hline
Total Y                                 & 6  & 7 & 8 \\ \hline
\end{tabular}}
\end{table}

==> preamble.tex <==
% \acmConference[ESEC/FSE 2023]{The 31st ACM Joint European Software Engineering Conference and Symposium on the
% Foundations of Software Engineering}{11 - 17 November, 2023}{San Francisco, USA}
%\documentclass[10pt,conference]{IEEEtran}
\usepackage{comment}
\usepackage{pifont}
\usepackage{pbox}
 \usepackage[flushleft]{threeparttable}
%\usepackage{natbib}
%\usepackage{amsmath,amssymb,amsfonts}

\usepackage{booktabs}

\usepackage{diagbox}
\usepackage{tablefootnote}

\usepackage{amsmath}
\usepackage{caption}


\usepackage{subcaption}


\usepackage{hyperref}
%\usepackage{algorithmic}
\usepackage{adjustbox}
\usepackage{multirow}
\usepackage{tabularx}
\usepackage{enumitem}
\usepackage{framed}
%\usepackage{lipsum}
\usepackage[linesnumbered,ruled,algo2e]{algorithm2e}
%\setcitestyle[square,numbers,compress]
\SetKwInput{KwInput}{Input} \SetKwInput{KwOutput}{Output} \SetKwInput{KwProcedure}{Procedure}
\newcommand\mycommfont[1]{\footnotesize\textcolor{blue}{#1}} \SetCommentSty{mycommfont}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage{graphicx}
\usepackage{textcomp}
\usepackage{xcolor}
\usepackage{multicol}
\usepackage{balance}
\usepackage{subcaption}
\usepackage{epstopdf}
\epstopdfDeclareGraphicsRule{.pdf}{png}{.png}{convert #1 \OutputFile} \AppendGraphicsExtensions{.pdf}
\usepackage{array}
% \usepackage{listings}
\definecolor{Gray}{gray}{0.9}
\definecolor{pgreen}{rgb}{0,0.5,0}
\newcommand{\charms}{Harms}
%\newcommand{\xmark}{\ding{55}}%
\usepackage{amsthm}
\makeatletter
\def\th@plain{%
  \thm@notefont{}% same as heading font
  \itshape % body font
}
\def\th@definition{%
  \thm@notefont{}% same as heading font
  \normalfont % body font
} \makeatother
\usepackage{capt-of}
\newtheorem{example}{Example}
\newtheorem{definition}{Definition}
\newtheorem{preposition}{Preposition}

\usepackage{color, colortbl}
\definecolor{grey}{rgb}{0.7,0.7,0.7}

%diff
\newcommand{\lstbg}[3][0pt]{{\fboxsep#1\colorbox{#2}{\strut #3}}}
\lstdefinelanguage{diff}{
  basicstyle=\ttfamily\scriptsize,,
  morecomment=[f][\lstbg{red!20}]-,
  morecomment=[f][\lstbg{green!20}]+,
  morecomment=[f][\lstbg{yellow!20}]++,
  morecomment=[f][\textit]{@@},
  texcl=false
}

\usepackage{tcolorbox}
% \usepackage{xcolor}
\definecolor{todocolor}{rgb}{0.9,0.1,0.1}
\definecolor{indiagreen}{rgb}{0.07, 0.53, 0.03}
\definecolor{hycolor}{rgb}{0.7,0.7,0.3}
\definecolor{darkbrown}{rgb}{0.4, 0.26, 0.13}


\newcommand*\justify{%
  \fontdimen2\font=0pt
  %\fontdimen2\font=0em% interword space
  \fontdimen3\font=0pt%0em% interword stretch
  \fontdimen4\font=0.1em% interword shrink
  \fontdimen7\font=0em% extra space
  \hyphenchar\font=`\-% allowing hyphenation
}
\newcommand{\nbc}[3]{
        {\colorbox{#3}{\scriptsize\textcolor{white}{#1}}}
            {\textcolor{#3}{\small$\blacktriangleright$\textit{#2}$\blacktriangleleft$}}
}

% \usepackage{listings}
\lstset{ captionpos=b, showspaces=false, showstringspaces=false, breaklines=true, frame=tb,framerule=0.1pt,
keywordstyle=\ttfamily\bfseries, commentstyle=\ttfamily\textit, escapechar=\^,
%frame=single,
texcl=true language=Java, basicstyle=\ttfamily\footnotesize, numbers=left, stepnumber=1, breakatwhitespace=false,
linewidth=\textwidth, xleftmargin=0.4cm, escapeinside={(*@}{@*)} }


% \usepackage{xcolor}
\definecolor{main-color}{rgb}{0.6627, 0.7176, 0.7764}
\definecolor{string-color}{rgb}{0.3333, 0.5254, 0.345}
\definecolor{key-color}{rgb}{0.8, 0.47, 0.196}

\lstdefinestyle{mystyle} {
    language = Java,
    basicstyle = {\ttfamily \color{main-color}},
    stringstyle = {\color{string-color}},
    keywordstyle = {\color{key-color}},
    keywordstyle = [2]{\color{lime}},
    keywordstyle = [3]{\color{yellow}},
    keywordstyle = [4]{\color{teal}},
    morekeywords = [3]{<<, >>},
    morekeywords = [4]{++},
    basicstyle=\ttfamily\scriptsize,
    commentstyle=\color{blue}\ttfamily,
    morecomment=[f][\lstbg{red!20}]-,
    morecomment=[f][\lstbg{green!20}]+,
    morecomment=[f][\lstbg{yellow!20}]++,
    morecomment=[f][\lstbg{yellow!20}]--,
    morecomment=[f][\textit]{@@},
    breaklines=false,
    texcl=false
}


\newcommand{\hsuNote}[1]{\nbc{HaiboNote}{#1}{indiagreen}}

\newcommand{\shinNote}[1]{\nbc{shinNote}{#1}{red}}


\newcommand{\hsu}[1]{\nbc{Haibo}{#1}{todocolor}}
\newcommand{\shin}[1]{\nbc{shin}{#1}{hycolor}}
\newcommand{\yulei}[1]{\nbc{Zhezhong}{#1}{hycolor}}
\newcommand{\huaien}[1]{\nbc{huaien}{#1}{blue}}

\newcommand{\cn}[1]{{\color{red}[cn: #1]}}
\setlength{\skip\footins}{3pt}

\lstnewenvironment{bash}[1][]
  {\lstset{language=[latex]TeX}\lstset{%
   numbers=left,numberstyle=\scriptsize,
   %stepnumber=1,numbersep=5pt,
   %framesep=5pt,
   %showstringspaces=false,
   commentstyle=\color{pgreen},
   xleftmargin=5pt,
   xrightmargin=5pt,
   aboveskip=\bigskipamount,
   belowskip=\bigskipamount, #1,
}} {}

\lstdefinestyle{testlstcolor}{
    language={sh},
    moredelim=**[is][\color{red}]{~}{~},
    moredelim=**[is][\color{blue}]{<}{>},
    moredelim=**[is][\bfseries]{***}{***},
    moredelim=**[is][\color{green}]{~~}{~~},
    showstringspaces=false,
    basicstyle=\ttfamily,
    literate={\\~}{{\textasciitilde}}1
        {\\<}{{\unichar{"003C}}}1
        {\\>}{{\unichar{"003E}}}1
}
%

%\newcommand{\consequences}{12}
\newcommand{\specialcell}[2][c]{%
  \begin{tabular}[#1]{@{}c@{}}#2\end{tabular}}
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\usepackage{tikz}

\usepackage{xspace}

\newcommand\cparagraph[1]{\noindent\textbf{#1.}\xspace}


\newcommand{\haibo}[1]{\nbc{haibo}{#1}{blue}}
\newcommand{\modifyhaibo}[1]{{\color{azure(colorwheel)}{#1}}}

\newcommand{\modifyhonghao}[1]{{\color{darkgreen}{#1}}}

==> problem-formulation.tex <==
\section{Related Work and Problem Formulation}
\label{sec:related}
%(given an input program, automatically generates a transformed program with less lines of code than the input program) (given an input program, automatically generates a transformed program with less lines of code than the input program) 



%\noindent\textbf{Importance of program transformations with reduced LOC.} 
%Program transformations that lead to reduced lines of code (LOC) play important roles  in (1) manual program transformations for software maintenance, and (2) automated techniques for debugging and testing.    For software maintenance, a recent study in Meta have motivated the importance of removing unnecessary code to respect users’ privacy expectations and help engineers to work efficiently~\cite{shackleton2023dead}. The framework used lines of code to measure code assets, and showed that removing unnecessary code enable the deletion of terabytes of data, saving over one megawatt of compute power due to removal of the corresponding processing pipelines.

Table~\ref{tab:Differences} highlights the differences between our work and prior techniques that produce programs of reduced sets.
The problem of \emph{automated program simplification} has been widely studied since 1965~\cite{nievergelt1965automatic}. 
We briefly discuss prior definitions of program simplification below:

\cparagraph{Syntactic program simplification} According to~\cite{nievergelt1965automatic}, syntactic program simplification refers to 
\emph{``simplifications which depend on the form of the program 
only, i.e. can be detected and proved to lead to an equivalent 
program without knowledge of what the program is supposed 
to do''}. This approach focuses on using a set of transformations known to preserve program equivalence. It is aligned with rule-based techniques (such as refactoring) in Table~\ref{tab:Differences}, where equivalent-preserving transformations are applied to enhance program design~\cite{becker1999refactoring}. Therefore, we define \emph{\textbf{syntactic program simplification}} as a way to obtain programs with fewer lines of code through semantic-preserving transformations. Typically, these techniques use static analysis to check for equivalence.


%Note that refactoring may or may not lead to programs with fewer lines of code but in this paper, we mainly study refactoring that leads to reduced lines of code.
%As this syntactic form 
%emphasizes using a well-designed set of transformations that are known to be equivalence-preserving; it is related to rule-based approaches in Table~\ref{tab:Differences} (e.g., \emph{refactoring} where equivalence-preserving program transformations are applied to improve the design of programs~\cite{becker1999refactoring}). 
%Hence, we define \emph{\textbf{syntactic program simplification}} as a technique where simplified programs (programs with fewer source lines of code) are obtained via transformations that are known to produce equivalence-preserving programs. These techniques usually rely on static analysis to check for equivalence. 

%Refactoring is way of restructuring code via semantic-preserving program transformations to improve the design of programs~\cite{becker1999refactoring}. 
Refactoring, a representative of syntactic program simplification has been widely studied where most studies focus on the refactoring practice ~\cite{peruma2022refactor,alomar2019can}. To reduce the time and effort in manual refactoring, many automated refactoring approaches have been proposed~\cite{gyori2013crossing,meng2015does}. Several approaches use refactoring to support code review ~\cite{alizadeh2019refbot,tsantalis2020refactoringminer}.

%\input{sections/differentrelatedwork}

%Some of the program transformations found in our study are commonly used in refactoring tools (e.g., lambda expressions ~\cite{gyori2013crossing,tsantalis2017clone}). The key difference between refactoring and \simpli{} is that it has the additional criterion that the resulting transformed program should be smaller (reduced lines of code), whereas refactoring does not necessarily lead to reduced code size. %(e.g.,  \texttt{Extract Local Variable}, one of the most popular refactoring according to a previous study ~\cite{negara2013comparative}, may even lead to an additional line of code due to the insertion of a new local variable). 
%As several program transformations studied are different from transformations supported by modern refactoring engines and our study shows that they are frequently used by developers, we hope that our study will inspire the introduction of new transformations into current refactoring engines.

\cparagraph{Semantic program simplification} Several automatic simplification techniques \emph{rely on test executions (e.g., test outcome) to check for behavioral equivalence to produce smaller programs} (we call them \emph{\textbf{semantic program simplification}})~\cite{ lu2012automatic,harman1995using,agrawal1990dynamic,ddmin,zhang2013practical,jiang2017simplydroid}. Semantic program simplification has been applied in many domains (e.g., simplifying event sequences~\cite{jiang2017simplydroid}, and deobfuscation~\cite{lu2012automatic}). 


In terms of transformations used, 
these techniques either rely on deletions (delta debugging) or obtain a reduced list of statements by focusing on a slicing criterion (dynamic slicing). We call them deletion-based approaches in Table~\ref{tab:Differences}. Several techniques use limited types of transformation (e.g., mutation and crossover operators for pixel shader simplification~\cite{shader}, \emph{remove} and \emph{move}
for debugging concurrent programs~\cite{jalbert2010trace}, replacing identifiers and subtrees of parse tree for program reduction~\cite{xu2023pushing}).
%a genetic algorithm approach uses mutation and crossover operators for pixel shader simplification~\cite{shader}., \texttt{Tinertia}, a heuristic trace simplification algorithm, uses \emph{remove} and \emph{move} simplifying operations for effective debugging of concurrent programs~\cite{jalbert2010trace}. 
These techniques usually rely on a variant of (1) delta debugging~\cite{ddmin}, and (2) dynamic slicing~\cite{agrawal1990dynamic,harman1995using,lu2012automatic}. 
Delta debugging increasingly deletes smaller parts of the input file and run tests to check if the simplified input changes the test outcome~\cite{ddmin}.
Dynamic slicing focuses on ``all statements that actually affect the value of a variable 
occurrence for a given program input''~\cite{agrawal1990dynamic}.  Our work is different from dynamic slicing or its variants (e.g., observation-based slicing~\cite{binkley2013observation}) in that: (1) slicing-based techniques isolate feature-related elements (e.g., statements) under certain criteria, whereas we focus on the program itself to obtain a smaller program (reduced LOC); (2) we obtain various behavior-preserving transformation types that beyond mere deletion for simplification. \emph{Our set of transformations can serve as the basis for providing more diverse candidates for delta debugging-based techniques to facilitate debugging.} Several researches focus on specific aspects of semantic program transformations, e.g., a prior work ~\cite{dyer2014mining} studied the actual and potential usage of Java language features. Another study~\cite{ramos2023melt} mined API migration rules from PRs. Gil et al.~\cite{gil2017spartanizer} introduced an Eclipse plugin named Spartanizer that helps developers apply refactoring. Higo et al.~\cite{higo2022constructing} constructed a dataset of functionally equivalent Java methods using automated test generation techniques. Different from these techniques, we focus on transformations that could result in simplified programs.



%Our paper different from all these approaches in that it seeks to study the set of program transformations used in \simpli{}. Instead of relying on mere deletions or mutation operators, we think that using a more diverse set of transformations may benefit prior approaches that rely on program simplification.
%


\cparagraph{Large language models for program transformation} Large language models (LLMs) have shown promising results in code-related tasks. Most prior learning-based approaches either focus on tasks like method name recommendations~\cite{parsa2023method}, code smell detection~\cite{azeem2019machine}, bug fixing~\cite{zhang2022coditt5}, reducing bug-triggering programs~\cite{zhang2024lpr} (via five predefined transformations) or proposing new objectives to improve the effectiveness of pre-training for LLMs of code~\cite{chakraborty2022natgen}. The most relevant techniques to us are the two general-purpose code transformation models: %\tufano{}~\cite{tufano2019learning} and \autotransform{}~\cite{thongtanunam2022autotransform}. Different from prior approaches, \tooln{} focuses on generating simplified programs with diverse transformations. 

%\cparagraph{\cpsimpli{}} As noted in prior work~\cite{nievergelt1965automatic}, during manual program simplification, developers usually have the required domain knowledge to produce semantically equivalent programs that are smaller. %(we call this \emph{\textbf{manual program simplification}}). Hence, there is no need to restrict the set of program transformations as in prior semantic program simplification techniques. In
%Hence, \emph{we study  \simpli{}} that combines the best of both worlds by including (1) syntactic program transformation, and (2) semantic program simplification. %We hypothesize that it uses a diverse set of semantically-equivalent program transformations to produce programs with less lines of code.  

During our study, we needed a clear definition for what
we consider a refactoring, and program simplification. We define them as follows:
% \todo{change, remove or update these definition}

% \begin{definition}[Refactoring]
% \label{def:ref}
% Refactoring is a set of \textbf{rule-based} equivalent-preserving program transformations that rely on a predefined set of \textbf{syntactic} program transformations. 
% \end{definition}

% change according to reviewer3's review comment
\begin{definition}[Harmful Content Coverage]
\label{def:ref}
Given a 
Refactoring is a set of equivalent-preserving program transformations that rely on a predefined set of \textbf{syntactic} program transformations. 
\end{definition}


As most refactoring engines only support making rule-based program transformations, we define refactoring in Def.~\ref{def:ref} to be rule-based transformations, which correspond to the refactoring types. To obtain the predefined set of rule-based equivalent-preserving transformations, we refer to the refactoring types listed in RefactoringMiner~\cite{tsantalis2020refactoringminer} and Martin Fowler’s refactoring catalog~\cite{becker1999refactoring}. As our goal is to obtain a broader and diverse set of program transformations commonly used by open-source developers when simplifying code, our study in Section~\ref{sec:study} investigated the developers' perspective of program simplification.

%\begin{definition}[Program Simplification]
%\label{def:ds}
%Program simplification is a set of equivalent-preserving program transformations that include both \textbf{syntactic} and \textbf{semantic} program transformations that lead to less Source Lines of Code (SLOC).
%\end{definition}


% \begin{definition}[\cpsimpli{}]
% \label{def:developersimp}
% \cpsimpli{} is program simplifications defined based on \textbf{developers' perception} of program simplifications (i.e., transformations that the developers considered as a way to ``simplify code''). \modifyshin{TODO: do we check for whether the transformation lead to less Source Lines of Code (SLOC) in the study? if yes, we need to add this as "as a way to simplify code, leading to less Source Lines of Code (SLOC)". Otherwise, we may remove the definition if we have consistent definition with the tool-supported ones}
% \end{definition}

% As our goal is to obtain a broader and diverse set of program transformations commonly used by open-source developers when simplifying code, our study in Section~\ref{sec:study} investigated the developers' perspective of program simplification.
% as defined in Definition~\ref{def:developersimp}.   


%rely on a predefined set of syntactic program transformations. 

%During manual program simplification, developers usually have the required domain knowledge to produce semantically equivalent programs that are smaller

%\cparagraph{\cpsimpli{}} As noted in prior work~\cite{nievergelt1965automatic}, during manual program simplification, developers usually have the required domain knowledge to produce semantically equivalent programs that are smaller, Hence, there is no need to restrict the set of program transformations as in prior semantic program simplification techniques. In
%Hence, \emph{we study  \simpli{}} that combines the best of both worlds by including (1) syntactic program transformation, and (2) semantic program simplification.

%\input{sections/relatedwork}
\begin{definition}[Test equivalent]
\label{def:test}
Given a pair of programs $(P, P')$ and a test suite $T$ executable in $P$ and $P'$, $P$ and $P'$ are test-equivalent if $\forall t_k \in T$  where each test $t_k$ takes as input $inp_k$ and produces output $out_k$, $P$($inp_k$)=$P'$($inp_k$)=$out_k$ (i.e., for all tests in $T$, $P$ and $P'$ produce the same outputs).%$O$ is the Oracle for the property to preserve with $O$(p) = true. We consider program $P$ and $P'$ as semantic-equivalent if $O$($P$) = true and $O$($P'$) = true.
\end{definition}


%(where $P'$ is obtained via a semantic-preserving transformation to $P$)



% \begin{definition}[Tool-supported Program Simplification]
% \label{def:tsimplification}
% Given a program $P$, and a transformed program $P'$, $P'$ is a program produced via tool-supported program simplification of $P$ if (1) $P'$ is obtained via \simpli{}, (2) $P'$ contains less Source Lines of Code (SLOC) than $P$, and (3) $P$ and $P'$ are test-equivalent. The transformed program $P'$ is obtained through a set of transformations, including (1) syntactic program transformations, and (2) semantic program simplifications. 
% \end{definition}




Although there are various granularity levels (e.g., statement, line, or character) used in prior techniques, we choose SLOC to represent simplified programs because it has been widely used in deletion-based~\cite{ddmin,hodovan2016modernizing} and rule-based approaches~\cite{dig2009refactoring}.
% \todo{check if you want to remove this line about the same SLOC less token} When the SLOCs remain the same, we consider the reduction in the number of tokens. 

%As our goal is to obtain a broader and diverse set of program transformations commonly used by open-source developers when simplifying code, our study in Section~\ref{sec:study} investigated the developers' perspective of program simplification as defined in Definition~\ref{def:developersimp}.
%As with existing code model~\cite{wang2021codet5}, our tool-supported program simplification currently only supports making method-level transformations. 











==> sec4-future.tex <==



\section{Future: Programming environment of 2030-35 and beyond}

%{\bf\em Writer: Abhik Roychoudhury, Shin Hwei Tan}


In the programming environment of 2030-35 where LLM-based auto-programming techniques have reached certain level of maturity, programmers may need to switch to different roles to fully utilize the power of auto-programming.

\begin{figure}
        \centering

\begin{tabular}{cc}
\begin{tabular}{c}
        \includegraphics[width =0.35\textwidth]{picture-composer.jpg}
\end{tabular} &
\begin{tabular}{c}
\includegraphics[width=0.35\textwidth]{qa.jpg}
\end{tabular}\\
(a) & (b) \\
\end{tabular}
        \caption{Evolution of programmer roles captured by DALL-E;
        programmer role (a) as code composer and designer instead of code writer, 
        (b) as quality assurance specialist instead of code writer.
        }\label{combined}
    \end{figure}

%\noindent\textbf{Adaptive selection of LLMs for various downstream tasks.} 
\paragraph*{Programmer as code composer and designer instead of code writer.} With the advancement of LLM-based auto-programming, many software maintenance tasks that require code writing can be automatically solved by invoking the appropriate LLMs. Figure~\ref{combined}(a) shows an AI-generated picture by Image Creator that uses DALL·E where programmers acts as code composer and designer instead of code writer. Instead of playing the traditional role of a programmer who meticulously writes code for solving different tasks, they can focus on tasks that require high-level understanding of the requirements (e.g., designing the overall structure of the program and tentative algorithms), allowing automated tools to select the most effective model for the relevant maintenance tasks in which relevant code will be automatically generated. As current techniques mainly focus on specializing LLMs for a specific downstream task of auto-coding (e.g., program repair, log statement, test generation) to improve the effectiveness for the given task, a future programming environment will intelligently predict and select the appropriate model to invoke based the context of the downstream task. There are two scenarios in which LLM-based auto-programming can change the future programming environment: (1) in an Integrated Development Environment (IDE) setting, (2) in a continuous integration (CI) workflow. For example, in the IDE setting that requires instant feedback from the auto-coding tool for efficient interaction, future techniques can design a lightweight tool that can automatically complete and suggest relevant code snippets based on the (1) current surrounding code and (2) the list of available tasks (e.g., suggest adding a JUnit test for the newly written Java method or adding a log statement before a graceful exit of a program).  Meanwhile, in a CI workflow, certain event that represents abnormal behavior of a software system (e.g., test failures, build failures) can automatically trigger the need for a software maintenance task (e.g., the need for a repair can be triggered after a test failure). In this scenario, more sophisticated techniques can be used to further confirm the validity of the trigger (e.g., to distinguish between test failure or flaky test). These techniques include program analysis techniques (such as symbolic execution), test generation techniques (based on code changes within a commit), and log analysis (program monitoring). 

 
\begin{figure}
        \centering
    \includegraphics[width=0.65\textwidth]{./figures/Lastmile.pdf}
        \vspace*{-0.05in}
        \caption{Automated repair of auto-generated code}\label{lastmile}
    \end{figure}
\vspace*{-0.05in}
\paragraph*{Programmer as quality assurance specialist.} Although many tasks can be automated, we foresee that concerns regarding the quality of the autogenerated code still remain. As some of the autogenerated code can be misaligned with the intention of the programmer, the programmer will need to play the role of a quality assurance specialist and spend more time in checking the validity of the generated code. Apart from using traditional testing and static analysis tools, more specialized automated program repair techniques can be designed (e.g., by referring to prior study~\cite{fan2023automated} that investigated the mistakes of auto-generated code) to reduce the time and effort involving in checking the quality of auto-generated code.  Figure~\ref{combined}(b) shows an AI-generated picture for programmer main role as quality assurance specialist.
Figure \ref{lastmile} shows a schematic that concretizes this last-mile improvement of autogenerated code $P$ produced from natural language description using a tool like Copilot. The autogenerated code may be subject to program repair guided by a given test suite $T$. However, the process of repair inspects or examines (either explicitly or implicitly) a domain of program edits --- trying to shrink the space of candidate edits which are suitable for improving program $P$. In this way, a repaired program $P'$ is generated from $P$. In the process of examining the domain of program edits (and presumably ruling out a lot of candidate edits), the program repair process generates many additional tests $T'$ over and above the test suite $T$ which was used to guide the program repair process. The oracle (or expected behavior) of these additional tests $T'$ can be obtained via some processing of the natural language description from which $P$ is derived.   The additional test inputs $T'$ (along with their oracles) can then serve as evidence of "correctness" of the repaired program $P'$.  We envision that code-generators of the future will not be only LLMs, but  LLM agents augmented with program analysis / repair capabilities. These augmented code generators may then try to commit code like human programmers, while submitting evidence in the form of generated tests $T'$ as evidence of correctness of (LLM-induced) code commits.  

\vspace*{-0.05in}
\paragraph*{Programmer-assisted safe auto-coding} %As there are prior incidents where using LLMs for auto-programming lead to leakage of sensitive data, programmers who would like to benefit from the power of LLM-based auto-programming will need to identify (and protect) the sensitive data before feeding them to LLMs. Existing code obfuscation techniques and data encryption algorithms can be used as a first layer of protection. %Figure~\ref{composer} shows an AI-generated picture for programmer-assisted automated programming. 
We envision that Large Language Model (LLM) generated code may be integrated into legacy code-bases of existing software projects. This could be in the form of libraries performing specific tasks, where the library code is generated with LLM. For safe integration of such LLM generated code in human-written software projects, one may need {\em sanitizer code} (e.g. \cite{asan}) so that the LLM generated code can be used by the bigger software project safely. Until we reach the stage of completely automating the generation of entire software projects, there may be a need to study (a) automated repair or improvement of LLM generated code, or (b) executing LLM generated code in a {\em contained} manner so that it can cause limited harm to the rest of the software system, or (c) generate verified LLM code whenever appropriate formal specifications are available. One first step towards verified LLM code can be to generate code in a programming language supporting verification ({\em e.g.}, see \cite{Misu24}). We could also generate both programs and proofs (about the program satisfying some formal properties) from LLMs. Such formal properties may be obtained from natural language, in which there is some work \cite{Mauro}. Automated generation of proofs from LLMs has also been recently studied \cite{Baldur}. All of these works provide impetus in moving towards higher assurance code from LLMs. 

\vspace*{-0.05in}
\paragraph*{Autonomous Program Improvement} We view the approach of program repair on unsafe code generated by LLMs to be a more {\em flexible} approach for automatically generating safe code (as it is based on code transformations), as compared to tuning or restriction of LLMs to generate safe outputs. Moving forward, researchers can examine this line of work, in addition to significant short-term efforts in prompt engineering and LLM tuning. Repair of the automatically generated code based on tests gives us more flexibility, partly because we can also choose the tests we use to guide the program repair. The repair as well as other tasks like feature addition can be achieved autonomously by LLM agents which are aware of the structure of the code. The recent work on AutoCodeRover \cite{acr} is an example work in this direction. In the near future, the focus will be to improve the efficacy of these agents. The combination of auto-coding from  natural language and autonomous software improvement using LLMs, is an enticing possibility which can be achieved by 2030. This would shift the role of a future software engineer towards achieving {\em assured autonomy} by focusing on {\em trust} of the autonomous artifacts, instead of engineering software systems at {\em scale}. The scale of software systems is likely to be achieved automatically in future, thus shifting the attention to \underline{\em trust}.

%If the LLM-generated code is subject to test generation (with test oracles derived from natural language descriptions), the tests can pinpoint errors which are then used to drive program repair. This workflow can be developed  on top of recent works like AutoCodeRover \cite{acr}.

%\vspace*{-0.05in}
\paragraph*{Looking even further} Autonomous improvement of automatically generated code need not be restricted to application level programming. We could examine the feasibility of automatically repairing probabilistic programs, which are generated automatically. Probabilistic  programming succinctly expresses statistical inference tasks on probabilistic models \cite{fose14}, and are supported in the back-end by machine learning frameworks like Pytorch \cite{pytorch}. Recently symbolic execution of probabilistic programs was proposed \cite{Voogd23} which raises the possibility of semantics-aware probabilistic program repair, after an initial LLM guided automated generation of  probabilistic program snippets. This line of work could help us progress towards automated self improvement of learning tasks,  a speculative direction of future research.


%\begin{figure}
%        \centering
%        \includegraphics[width =0.35\textwidth]{collaboraterobot.jpg}
%        \caption{Programmer-assisted safe automated programming}\label{composer}
%    \end{figure}

%\noindent\textbf{Integrating auto-generated code into human-written code?} TODO : % legacy code

%- maybe move to the last mile improvement\noindent\textbf{Program Comprehension aided by programming environment?} TODO: adding a new feature or bug fix to understand code/ for software evolution with help of program analysis

%-maybe move to the explanability section


